When Image Denoising Meets High-Level Vision Tasks: A Deep Learning Approach

Conventionally, image denoising and high-level vision tasks are handled separately in computer vision. In this paper, we cope with the two jointly and explore the mutual influence between them. First we propose a convolutional neural network for image denoising which achieves the state-of-the-art performance. Second we propose a deep neural network solution that cascades two modules for image denoising and various high-level tasks, respectively, and use the joint loss for updating only the denoising network via back-propagation. We demonstrate that on one hand, the proposed denoiser has the generality to overcome the performance degradation of different high-level vision tasks. On the other hand, with the guidance of high-level vision information, the denoising network can generate more visually appealing results. To the best of our knowledge, this is the first work investigating the benefit of exploiting image semantics simultaneously for image denoising and high-level vision tasks via deep learning. The code is available online https://github.com/Ding-Liu/DeepDenoising.

==> related.tex <==
\section{Related Work}



%\input{denoisingSurvey.tex}

Denoising is the task of estimating the high-quality signal from its noisy measurements. 
%Despite today's vast improvement in camera sensors, videos captured at high speed and in low light conditions are still corrupted by severe noise due to high sensitivity (\ie ISO) among other reasons. 
%The problem of noise in multimedia data is gaining prominence with the ubiquitous use of relatively low-quality camera sensors in smart phones and other devices {\color{red} help me think of some scenarios...}.
Classical image denoising methods take advantage of local or non-local structures presented in the image explicitly.
Natural images are well-known to be patch-wise sparse or compressible in transform domain, or over certain dictionary. 
Prior works \cite{Aharon2006,zoran2011learning,wen2015octobos} exploit such local structures and reduce noise by coefficient shrinkage for image restoration. 
%Apart from the image local properties, 
The later approaches, including SSC \cite{Mairal2009}, CSR \cite{Dong2011}, NCSR \cite{NCSR}, GSR \cite{zhang2014group}, WNNM \cite{WNNM}, PCLR \cite{PCLR}, PGPD \cite{PGPD}, STROLLR \cite{wen2017strollr}, as well as BM3D \cite{dabov2007image} and its extension for color images CBM3D~\cite{dabov2007color} -- group similar patches within the image globally via block matching or clustering, and impose non-local structural priors on these groups, which usually lead to state-of-the-art image denoising performance.


% Review of deep based denoising methods:
More recently, the popular deep neural network techniques have been applied to low-level vision tasks.
Specifically, a number of deep learning models have been developed for image denoising~\cite{vincent2008extracting,jain2009natural,burger2012image,xie2012image,mao2016image,kim2017deeply},
which can be classified into two categories:    multi layer perception (MLP) based models and convolutional neural network (CNN) based models. 
Early MLP based models for image denoising include the stacked denoising autoencoder~\cite{vincent2008extracting,xie2012image}.
%which is an extension of the stacked autoencoder originally designed for unsupervised feature learning.
%A denoising autoencoder is proposed for both image denoising and blind image inpainting by Xie et al.~\cite{xie2012image}.
Burger et al.\ \cite{burger2012image} introduce a plain multilayer perception (MLP) and thoroughly compare its denoising performance with 
%a state-of-the-art denoising algorithm, 
BM3D~\cite{dabov2007image} in different experimental settings.
CNNs are first utilized for image denosing by Jain and Seung~\cite{jain2009natural}.
Recent works \cite{SF,TRND} attempt to unfold the iterative algorithms, and construct a cascaded convolutional filtering architecture for image denoising.
%Mao et al.~\cite{mao2016image} propose a very deep convolutional autoencoder for image restoration and exploit skip connections for better gradient propagation during training, which achieves superior performance over other recent methods.
Very deep networks are adopted with skip connections for image restoration~\cite{mao2016image,zhang2017beyond}, which achieve superior performance over other recent methods.
Dilated convolutions are exploited to learn the residual image for denoising in \cite{zhang2017learning}.
